On Inherent Adversarial Robustness of Active Vision Systems

Current Deep Neural Networks are vulnerable to adversarial examples, which alter their predictions by adding carefully crafted noise. Since human eyes are robust to such inputs, it is possible that the vulnerability stems from the standard way of processing inputs in one shot by processing every pixel with the same importance. In contrast, neuroscience suggests that the human vision system can differentiate salient features by (1) switching between multiple fixation points (saccades) and (2) processing the surrounding with a non-uniform external resolution (foveation). In this work, we advocate that the integration of such active vision mechanisms into current deep learning systems can offer robustness benefits. Specifically, we empirically demonstrate the inherent robustness of two active vision methods - GFNet and FALcon - under a black box threat model. By learning and inferencing based on downsampled glimpses obtained from multiple distinct fixation points within an input, we show that these active methods achieve (2-3) times greater robustness compared to a standard passive convolutional network under state-of-the-art adversarial attacks. More importantly, we provide illustrative and interpretable visualization analysis that demonstrates how performing inference from distinct fixation points makes active vision methods less vulnerable to malicious inputs.

==> Introductions/old_introduction.tex <==
%Adversarial inputs are crafted by carefully adding noise to images, often imperceptible or irrelevant to the human eye. This exploits vulnerabilities in standard deep neural networks, which process images passively in one shot. In contrast, the human perceptual system, as evidenced by neuroscience, can understand salient features of an object by switching between multiple fixation points (saccades) in an image and focusing on details when encountering relevant information (foveation). In this work, we advocate for integrating such active learning mechanisms into current deep learning systems. We empirically demonstrate that learning from multiple fixation points inherently enhances robustness in deep learning models. In a black-box threat model setup we evaluate the inherent robustness properties of two such active vision methods --- Glance and Focus Networks, and FALcon. We demonstrate how mechanisms such as glimpse-based learning at a downsampled resolution from multiple distinct fixation points contribute to the innate robustness of such methods against state-of-the-art adversarial attacks. This results in achieving \textbf{2-3} times greater robustness compared to a standard passive convolutional network. We further provide illustrative and interpretable visualizations. These show how active vision methods, during inference primed by their initial glimpse based on distinct fixation points, are less vulnerable to malicious inputs. %R-Blur/R-Warp utilize a single random fixation point per image during training whereas "active" vision method involves learning from multiple distinct fixation points, resulting in a more robust comprehension of objects.   



%% Summary - Paragraph 1 talks about adversarial samples and the adversarial defense from the deep learning perspective.
Since the last decade deep learning has seen tremendous progress in a plethora of applications \cite{AlexNet, FasterRCNN, MRCNN, dosovitskiy2021an, GANs, rombach2022high}. However, these networks are susceptible to adversarial inputs, carefully crafted by adding noise that is imperceptible or ignored by human eyes \cite{szegedy2014intriguing, GoodfellowSS14, Papernot2016PracticalBA}. These malicious inputs have been shown to be detrimental to various vision-oriented applications \cite{Athalye2017SynthesizingRA,Hosseini2018SemanticAE,Joshi2019SemanticAA}. To circumvent the effect of such malicious attacks, several defense methods have been proposed, of which Adversarial Training (Adv-T)~\cite{madry2018towards} and Randomized Smoothing (RS)~\cite{RSmoothing} are the most prominent approaches. Although effective against adversarial attacks, the former is computationally expensive while the latter faces scalability issues necessitating the development of other sophisticated methods \cite{andriushchenko2020understanding, CutMix, li2023data, MoosaviDezfooli2018RobustnessVC, yue2023revisiting, zhang2018mixup}. Furthermore, these defense methods are developed purely based on the statistical and computational principles of deep learning. 
%% Summary - Paragraph 2 talks about human peripheral vision and its incorporation to passive vision methods. This is applying blurring and other effects to the input. We do not talk about the active vision here. That we introduce in the next paragraph.


In contrast, the human peripheral vision, which encompasses the outer edges of our visual field, is less sensitive to fine details and subtle variations in the image. As a result, noise added to the periphery of an image may go unnoticed or be considered insignificant by the human visual system. Thus, there is a growing interest in modeling bio-inspired peripheral vision with current vision methods for adversarial robustness. These include mechanisms such as cortical and retinal fixations \cite{Poggiocortical}, peripheral blurring \cite{shah2023training}, primal visual cortex processing \cite{VOneBlock} or fovea-based texture transformation \cite{gant2021evaluating}. As discussed in R-Blur \cite{shah2023training} most of these methods model the bio-inspired visual mechanics based on a single fixation point around the input during training.  
%% Summary - Paragraph 3 introduces the human active vision system. Going beyond than just modifying the input to model the peripheral vision. Active vision has both foveation and saccades coupled together. Such as in FALcon. foveate, switch and foveate again. And in this paragraph we only talk about the middle column of the figure. Paragraph 2 was peripheral vision. This more about the active vision system. 


The human perceptual system on the other hand, as evidenced by neuroscience \cite{curcio1990human, eckstein2011visual, land2012animal}, has a fundamentally different approach to perceiving and processing visual inputs. This entails an "active" process of shifting between various pertinent fixation points (Saccades) within a visual scene, followed by selectively attending to the most pertinent areas with varying detail (Foveation) centered around these fixation points. As a result, this aids in understanding the most salient aspects of the input for a given task while disregarding redundant or less relevant details in a cluttered environment, leading to inherent robustness. In this work, we advocate the integration of "active" vision into current deep learning methods that can lead to a robust learning representation. To support our argument, we consider two previous approaches—FALcon \cite{ibrayev2023exploring} and Glance and Focus Networks \cite{GFNet_2020}. Developed for distinct perception tasks, both demonstrate coupled mechanisms for assessing and focusing on relevant input portions as core components of their learning as described in the middle column of Figure~\ref{fig:block}. FALcon \textbf{(B)}, guided by Weakly Supervised Object Localization, assigns importance to \textit{predefined} fixation points based on "objectness" and progressively expands until successfully localizing the object or switching to another fixation point. In contrast, GFNet \textbf{(A)}, designed for image classification, determines a relevant fixation point through a glance step and focuses on high-resolution portions through subsequent focus step, stopping when sufficiently confident of the correct class. %Both approaches mimic the active natural vision of the human visual system, albeit with differing designs tailored for different tasks.

\begin{figure}[tb]
  \centering
  \includegraphics[height=6.5 cm]{Images/Block_ECCV_refined.png}
  \caption{Figure illustrates two methods of processing an adversarial input -- a passive method and an active method. The highlighted yellow box serves as a visual illustration of an adversarial sticker. \textbf{Left column:} One of the probable causes of passive methods being susceptible to adversarial inputs is the uniform processing : that means processing each pixel with same importance. \textbf{Middle column:} In contrast, active vision methods \textbf{(A) GFNet} and \textbf{(B) FALcon} learn the salient features of an object by observing it from multiple distinct fixation points via sequence of glimpses as indicated by the blue boxes. \textbf{Right column:} As a result, during inference, this leads to distinct predictions for the same image not all of which are affected by the adversarial noise.          
  }
  \label{fig:block}
\end{figure}

%% Summary - Paragraph 4 answers the why. Why do we hypothesize that learning from multiple points lead to inherent robustness. 
In this work, we empirically demonstrate that by performing inference from multiple fixation points, the active vision methods offer inherent robustness to adversarial samples in a black-box scenario compared to the passive baseline methods. The idea stems from the fact that the generated adversarial noise perturbs the input in a non-uniform manner, owing to imperceptibility conditions. Since Active vision methods focus on different portions of an input, this allows them to make multiple predictions. Due to the non-uniformity of adversarial noise, distinct fixation points result in different sequences of observations. As a result, these multiple predictions exhibit varying susceptibility to the attack. For example, as shown in the right-most column of Figure~\ref{fig:block}, FALcon makes two distinct predictions from two corresponding fixation points (red and blue dots). While the red fixation point results in a misprediction, the prediction from the blue point is consistently robust. This example illustrates how active vision methods can avoid the adversarial noise \footnote{We visually depict an adversarial sticker and generate adversarial samples using various attacks in our experiments, which are not limited to a few pixels in the image.}.


%% Summary 
To summarize, the main objective of this work is to study and understand the inherent robustness of the aforementioned active vision methods. A vanilla black-box threat model appears to be a suitable and fair evaluation protocol for these methods. In a black-box threat model, the attacker is unaware of the details of the underlying neural network. This allows us to examine the salient properties of such active vision methods that contribute to their inherent robustness while exposing them to adversarial samples in a consistent manner. We highlight our contributions as follows:


\begin{itemize}
    \item We provide a novel analysis of the inherent robustness of Active Vision Methods in a black box threat model setup.
    \item We empirically demonstrate the superior performance of these methods over standard passive baselines against SOTA adversarial attacks, achieving robustness up to \textbf{$(2-3)$} times as measured by accuracy under attack.  (\ref{ssec:blackbox}). %Similar performance enhancements are noticed for SOTA transfer attacks as well. (\ref{sssec:lgv}), (\ref{sssec:tgr})
    \item Through both quantitative and qualitative analyses, we showcase the salient learning aspects of these methods that contribute to their inherent robustness. These include glimpse-based learning in a downsampled resolution (\ref{ssec:glimpses}) and inference from distinct fixation points (\ref{ssec:saccades}). 
    \item We show visualizations interpreting how these methods triumph with remarkable resilience against adversarial samples, surpassing their corresponding baselines  (\ref{ssec:saccades}),(\ref{sssec:viz})
\end{itemize}

Please note that we do not propose an adversarial defense approach. Instead, we advocate natural active learning similar to a human visual system of such methods as the core reason for their inherent robustness without the need for additional adversarial training. The rest of the paper is structured as follows. In Section~\ref{sec:related} we discuss the relevant related work on active vision methods, bio-inspired adversarial defense, and transfer attacks. In Section~\ref{sec:avm}, we provide high-level overviews of the inference techniques adopted by GFNet \cite{GFNet_2020} and FALcon \cite{ibrayev2023exploring}. In Section~\ref{sec:method} we outline the black-box threat model and the metrics chosen to measure the robustness of active and passive methods. In Section~\ref{sec:exps}, we provide an extensive robustness study to highlight the inherent robustness of active vision methods both via qualitative and quantitative results. 

==> Tables/GeometricAttack.tex <==
% \setlength{\tabcolsep}{8pt}
\begin{table}[t!]
\centering
\caption{Geometric Attack using ResNet50 as surrogate.}
\label{tab:LGV_table}
\begin{tabular}{|c|l|cc|}
\hline
\multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{2}{c|}{Attack (LGV+)} \\ \cline{3-4} 
    &   & \multicolumn{1}{c|}{PGD} & BIM \\ \hline \hline
ResNet50 & 75.30 & \multicolumn{1}{c|}{3.50} & 2.40 \\ \hline 
Adv-T &  50.60 & \multicolumn{1}{c|}{50.20} & 49.80 \\ \hline
CutMix & 77.20 & \multicolumn{1}{c|}{13.10} &  10.0 \\ \hline
FALcon & 75.0 & \multicolumn{1}{c|}{34.70} & 29.60\\ \hline
GFNet & 74.20 & \multicolumn{1}{c|}{49.0} &   44.70 \\ \hline
\end{tabular}
\end{table}
\setlength{\tabcolsep}{6pt} % reverse back to Default -- 6pt
%%%% Original
% \begin{table}[t!]
% \caption{Geometric Attack}
% \label{tab:LGV_table}
% \begin{tabular}{|c|c|l|cc|}
% \hline
% \multirow{2}{*}{Surrogate} & \multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{2}{c|}{Attack}                \\ \cline{4-5} 
%                            &                         &                        & \multicolumn{1}{c|}{LGV + PGD} & LGV + BIM \\ \hline
% \multirow{5}{*}{ResNet50}  & ResNet50                & 75.30                  & \multicolumn{1}{c|}{3.50}      & 2.40      \\ \cline{2-5} 
%                            & Adv-T                   &  50.60                      & \multicolumn{1}{c|}{50.20}          &     49.80      \\ \cline{2-5} 
%                            & R-Blur                  &                        & \multicolumn{1}{c|}{}          &           \\ \cline{2-5} 
%                            & FALcon                  &                        & \multicolumn{1}{c|}{}          &           \\ \cline{2-5} 
%                            & GFNet                   &      74.20                 & \multicolumn{1}{c|}{49.0}          &   44.70        \\ \hline
% \end{tabular}
% \end{table}



==> Tables/GeometricAttack_TokenGradientRegularization.tex <==
% \def\arraystretch{1.2}% 
\begin{table}[!htb]
    % \caption{Global caption}
    \begin{minipage}{.5\linewidth}
    \centering
    \captionsetup{justification=centering}
    % \caption{Geometric Attack using ResNet50 as surrogate.}
    % \label{tab:LGV_table}
    % \begin{tabular}{|c|l|cc|}
    % \hline
    % \multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{2}{c|}{Attack (LGV+)} \\ \cline{3-4} 
    %     &   & \multicolumn{1}{c|}{PGD} & BIM \\ \hline \hline
    % ResNet50 & 75.30 & \multicolumn{1}{c|}{3.50} & 2.40 \\ \hline 
    % Adv-T &  50.60 & \multicolumn{1}{c|}{50.20} & 49.80 \\ \hline
    % R-Blur &  & \multicolumn{1}{c|}{} & \\ \hline
    % FALcon & & \multicolumn{1}{c|}{} & \\ \hline
    % GFNet & 74.20 & \multicolumn{1}{c|}{49.0} &   44.70 \\ \hline
    % \end{tabular}
   \includegraphics[width=\columnwidth]{Images/Geometric_attack.png}
    \captionof{figure}{Geometric Attack using ResNet50 as surrogate}
    \label{fig:LGV_table}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
          \captionsetup{justification=centering}
\caption{Token Gradient Regularization.}
\label{tab:TGR-table}
\begin{tabular}{|c|c|ccc|}
\hline
\multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{3}{c|}{Surrogate}                                                             \\ \cline{3-5} 
                        &                        & \multicolumn{1}{c|}{ViT-B/16 \cite{dosovitskiy2021an}}       & \multicolumn{1}{c|}{CaiT-S/24 \cite{Touvron2021GoingDW}}      & PiT-B \cite{Heo2021RethinkingSD}         \\ \hline \hline
ResNet50 \cite{He2015DeepRL}                & \textbf{93.10}                  & \multicolumn{1}{c|}{32.0}           & \multicolumn{1}{c|}{13.3}           & 10.30          \\ \hline
Adv-T \cite{madry2018towards}                  & 28.80                  & \multicolumn{1}{c|}{27.70}          & \multicolumn{1}{c|}{26.90}          & 26.90          \\ \hline
R-Blur \cite{shah2023training}                 &                        & \multicolumn{1}{c|}{}               & \multicolumn{1}{c|}{}               &                \\ \hline
Swin-v2 \cite{SwinV2}                & 99.00                  & \multicolumn{1}{c|}{31.10}          & \multicolumn{1}{c|}{10.3}           & 12.30          \\ \hline
RVT \cite{Mao2021TowardsRV}                    & 97.70                  & \multicolumn{1}{c|}{34.40}          & \multicolumn{1}{c|}{12.1}           & \textbf{14.50} \\ \hline
Adv-RVT \cite{Mao2021TowardsRV}               & 53.40                  & \multicolumn{1}{c|}{47.80}          & \multicolumn{1}{c|}{46.30}          & 45.70          \\ \hline
Focal Net  \cite{yang2022focal}             & \textbf{99.20}         & \multicolumn{1}{c|}{\textbf{35.60}} & \multicolumn{1}{c|}{13.20}          & 7.00           \\ \hline
FALcon \cite{ibrayev2023exploring}                 & 85.4                   & \multicolumn{1}{c|}{21.00}          & \multicolumn{1}{c|}{\textbf{15.10}} & 10.50          \\ \hline
GFNet  \cite{huang2022glance}                 & 89.5                   & \multicolumn{1}{c|}{\textbf{35.00}} & \multicolumn{1}{c|}{\textbf{22.5}}  & \textbf{15.80} \\ \hline
\end{tabular}
    \end{minipage} 
\end{table}

==> Tables/MultipleFixations.tex <==
\begin{table}[t!]
\caption{Effects of Inference from Multiple Fixation Points}
\label{tab:multiple_pred}
\begin{tabular}{|c|c|cc|}
\hline
\multirow{2}{*}{Surrogate} & \multirow{2}{*}{Target} & \multicolumn{2}{c|}{Attack}                          \\ \cline{3-4} 
                           &                         & \multicolumn{1}{c|}{PGD}            & MIM            \\ \hline
\multirow{3}{*}{ResNet34}  & ResNet50                & \multicolumn{1}{c|}{31.46}          & 20.20          \\ \cline{2-4} 
                           & FALcon (Top-1)          & \multicolumn{1}{c|}{49.83}          & 37.01          \\ \cline{2-4} 
                           & FALcon (Any)            & \multicolumn{1}{c|}{\textbf{54.37}} & \textbf{41.40} \\ \hline
\end{tabular}
\end{table}

==> Tables/PredictionPrecision.tex <==
\begin{table}[t!]
\caption{Precision of predictions.}
\label{tab:Fixation_PM_tab}
\begin{tabular}{|c|c|c|c|}
\hline
Samples           & Potential & Correct & Precision \\ \hline
Clean             & 25444 & 22740 & 0.89          \\ \hline
PGD & 18931  & 13603 & 0.72          \\ \hline
MIM & 16729  & 9160 & 0.55          \\ \hline
\end{tabular}
\end{table}

==> Tables/PredictionPrecision_MultipleFixation.tex <==
\begin{table}[!t]
    % \caption{Global caption}
    \begin{minipage}{.5\linewidth}
    \centering
    % \captionsetup{justification=centering}
    % \caption{Precision of predictions.}
    % \label{tab:Fixation_PM_tab}
    % % \scriptsize
    % \begin{tabular}{|c|c|c|c|}
    % \hline
    % Samples & Potential & Correct & Precision \\ \hline \hline
    % Clean & 25444 & 22740 & 0.89 \\ \hline
    % PGD & 18931  & 13603 & 0.72 \\ \hline
    % MIM & 16729  & 9160 & 0.55 \\ \hline
    % \end{tabular}
   \includegraphics[width=\columnwidth]{Images/Prec_of_Prediction.png}
    \captionof{figure}{Precision of predictions}
    \label{fig:Fixation_PM_tab}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
      \captionsetup{justification=centering}
    \caption{Effects of Inference from Multiple Fixation Points using ResNet34 as surrogate.}
    \label{tab:multiple_pred}
    % \begin{tabular}{|c|c|cc|}
    % \hline
    % \multirow{2}{*}{Surrogate} & \multirow{2}{*}{Target} & \multicolumn{2}{c|}{Attack}                          \\ \cline{3-4} 
    %                            &                         & \multicolumn{1}{c|}{PGD}            & MIM            \\ \hline \hline
    % \multirow{3}{*}{ResNet34}  & ResNet50                & \multicolumn{1}{c|}{31.46}          & 20.20          \\ \cline{2-4} 
    %                            & FALcon (Top-1)          & \multicolumn{1}{c|}{49.83}          & 37.01          \\ \cline{2-4} 
    %                            & FALcon (Any)            & \multicolumn{1}{c|}{\textbf{54.37}} & \textbf{41.40} \\ \hline
    % \end
    % \scriptsize
    \begin{tabular}{|c|cc|}
    \hline
    \multirow{2}{*}{Target} & \multicolumn{2}{c|}{Attack} \\ \cline{2-3} 
        & \multicolumn{1}{c|}{PGD} & MIM \\ \hline \hline
    ResNet50 & \multicolumn{1}{c|}{31.46} & 20.20 \\ \hline 
    FALcon (Top-1) & \multicolumn{1}{c|}{49.83} & 37.01 \\ \hline
    \cellcolor{Ours} \textbf{FALcon (Any)} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{54.37}} & \cellcolor{Ours} \textbf{41.40} \\ \hline
    \end{tabular}
    \end{minipage} 
\end{table}

==> Tables/TokenGradientRegularization.tex <==
\begin{table}[t!]
\centering
\caption{Token Gradient Regularization.}
\label{tab:TGR-table}
\begin{tabular}{|c|c|ccc|}
\hline
\multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{3}{c|}{Surrogate}                                                             \\ \cline{3-5} 
                        &                        & \multicolumn{1}{c|}{ViT-B/16 \cite{dosovitskiy2021an}}       & \multicolumn{1}{c|}{CaiT-S/24 \cite{Touvron2021GoingDW}}      & PiT-B \cite{Heo2021RethinkingSD}         \\ \hline \hline
ResNet50 \cite{He2015DeepRL}                & \textbf{93.10}                  & \multicolumn{1}{c|}{32.0}           & \multicolumn{1}{c|}{13.3}           & 10.30          \\ \hline
Adv-T \cite{madry2018towards}                  & 28.80                  & \multicolumn{1}{c|}{27.70}          & \multicolumn{1}{c|}{26.90}          & 26.90          \\ \hline
R-Blur \cite{shah2023training}                 &                        & \multicolumn{1}{c|}{}               & \multicolumn{1}{c|}{}               &                \\ \hline
Swin-v2 \cite{SwinV2}                & 99.00                  & \multicolumn{1}{c|}{31.10}          & \multicolumn{1}{c|}{10.3}           & 12.30          \\ \hline
RVT \cite{Mao2021TowardsRV}                    & 97.70                  & \multicolumn{1}{c|}{34.40}          & \multicolumn{1}{c|}{12.1}           & \textbf{14.50} \\ \hline
Adv-RVT \cite{Mao2021TowardsRV}               & 53.40                  & \multicolumn{1}{c|}{47.80}          & \multicolumn{1}{c|}{46.30}          & 45.70          \\ \hline
Focal Net  \cite{yang2022focal}             & \textbf{99.20}         & \multicolumn{1}{c|}{\textbf{35.60}} & \multicolumn{1}{c|}{13.20}          & 7.00           \\ \hline
FALcon \cite{ibrayev2023exploring}                 & 85.4                   & \multicolumn{1}{c|}{21.00}          & \multicolumn{1}{c|}{\textbf{15.10}} & 10.50          \\ \hline
GFNet  \cite{huang2022glance}                 & 89.5                   & \multicolumn{1}{c|}{\textbf{35.00}} & \multicolumn{1}{c|}{\textbf{22.5}}  & \textbf{15.80} \\ \hline
\end{tabular}
\end{table}

==> Tables_App/Inherent_Robustness.tex <==
\def\arraystretch{1.2}%
\begin{table}[t!]
\centering
\caption{Inherent Robustness of Active Vision Methods\vspace{-2mm}}
\label{tab:Main}
\begin{tabular}{c|c|cccc|}
% \cline{2-6}
% ~ for no line in one cell; 
% | for corner
% *4- for cline for 4 cells
\hhline{~|*5{-}|}
 & \cellcolor{Gray} & \multicolumn{1}{c|}{\cellcolor{Gray}ResNet50 \cite{He2015DeepRL}} & \multicolumn{1}{c|}{\cellcolor{Gray}Adv-T$\star$ \cite{madry2018towards} } & \multicolumn{1}{c|}{\cellcolor{Gray}\textbf{FALcon\cite{ibrayev2023exploring}}} & \cellcolor{Gray}\textbf{GFNet \cite{huang2022glance}} \\ \hhline{~~|*4{-}|}
 % \cline{3-6} 
 
\multirow{-2}{*}{} & \multirow{-2}{*}{\cellcolor{Gray}\textbf{Clean}} & \multicolumn{1}{c|}{\cellcolor{Gray}76.15} & \multicolumn{1}{c|}{\cellcolor{Gray}47.91} & \multicolumn{1}{c|}{\cellcolor{Gray}\textbf{72.97}} & \cellcolor{Gray}\textbf{75.88} \\ \hhline{~|*5{-}|} \noalign{\vspace{0.35ex}} \hline

% &  \multirow{2}{*}{Clean}  & \multicolumn{1}{c|}{ResNet50  }  & \multicolumn{1}{c|}{Adv-T} & \multicolumn{1}{c|}{FALcon } & GFNet \\ \cline{3-6} 
  % &  & \multicolumn{1}{c|}{76.15}  & \multicolumn{1}{c|}{47.91} & \multicolumn{1}{c|}{72.97}  & 75.88   \\ \hline \hline
  
\multicolumn{1}{|c|}{\multirow{2}{*}{Surrogate}} & \multirow{2}{*}{Target} & \multicolumn{4}{c|}{Attack} \\ \cline{3-6}   

\multicolumn{1}{|c|}{} &  & \multicolumn{1}{c|}{PGD \cite{madry2018towards}}   & \multicolumn{1}{c|}{MIM \cite{MIM}}    & \multicolumn{1}{c|}{VMI \cite{VMI}}    & P-IFGSM \cite{GaoZhang2020PatchWise} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{ResNet34 \cite{He2015DeepRL}}}  & ResNet50  & \multicolumn{1}{c|}{31.46} & \multicolumn{1}{c|}{20.20}  & \multicolumn{1}{c|}{11.61}  & 31.62   \\ \cline{2-6} 

\multicolumn{1}{|c|}{} & Adv-T$\star$ & \multicolumn{1}{c|}{47.63} & \multicolumn{1}{c|}{47.37}  & \multicolumn{1}{c|}{47.16}  & 46.94   \\ \hhline{~|*5{-}|}
% \cline{2-6} 

\multicolumn{1}{|c|}{} & \cellcolor{Ours}\textbf{FALcon} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{49.83}} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{37.01}}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{29.40}}  & \cellcolor{Ours} \textbf{40.46}   \\ \hhline{~|*5{-}|}
% \cline{2-6} 

\multicolumn{1}{|c|}{} & \cellcolor{Ours} \textbf{GFNet}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{57.82}} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{48.60}}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{41.17}}  & \cellcolor{Ours} \textbf{46.93} \\ \hline \hline
%% Uncolored -- 
% \multicolumn{1}{|c|}{} & \textbf{FALcon} & \multicolumn{1}{c|}{\textbf{49.83}} & \multicolumn{1}{c|}{\textbf{37.01}}  & \multicolumn{1}{c|}{\textbf{29.40}}  & \textbf{40.46}   \\ \cline{2-6} 

% \multicolumn{1}{|c|}{} & \textbf{GFNet}  & \multicolumn{1}{c|}{\textbf{57.82}} & \multicolumn{1}{c|}{\textbf{48.60}}  & \multicolumn{1}{c|}{\textbf{41.17}}  & \textbf{46.93} \\ \hline \hline
    
\multicolumn{1}{|c|}{\multirow{4}{*}{ResNet50 \cite{He2015DeepRL}}}  & ResNet50               & \multicolumn{1}{c|}{0.00}  & \multicolumn{1}{c|}{0.00}   & \multicolumn{1}{c|}{0.00}   & 0.00    \\ \hhline{~|*5{-}|}
% \cline{2-6} 
    
\multicolumn{1}{|c|}{} & Adv-T$\star$  & \multicolumn{1}{c|}{47.68} & \multicolumn{1}{c|}{47.36}  & \multicolumn{1}{c|}{47.22}  & 46.83   \\ \hhline{~|*5{-}|}
% \cline{2-6}    

\multicolumn{1}{|c|}{} & \cellcolor{Ours} \textbf{FALcon}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{37.54}} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{19.96}}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{12.07}}  &   \cellcolor{Ours} \textbf{27.37}      \\ \hhline{~|*5{-}|}
% \cline{2-6} 
    
\multicolumn{1}{|c|}{} & \cellcolor{Ours} \textbf{GFNet} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{51.85}} & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{42.16}}  & \multicolumn{1}{c|}{\cellcolor{Ours} \textbf{32.33}}  & \cellcolor{Ours} \textbf{43.33}   \\ \hline
% % Colored-
% \multicolumn{1}{|c|}{} & \textbf{FALcon}  & \multicolumn{1}{c|}{\textbf{37.54}} & \multicolumn{1}{c|}{\textbf{19.96}}  & \multicolumn{1}{c|}{\textbf{12.07}}  &   \textbf{27.37}      \\ \cline{2-6} 
    
% \multicolumn{1}{|c|}{} & \textbf{GFNet} & \multicolumn{1}{c|}{\textbf{51.85}} & \multicolumn{1}{c|}{\textbf{42.16}}  & \multicolumn{1}{c|}{\textbf{32.33}}  & \textbf{43.33}   \\ \hline

\end{tabular}
%% Older with R-Blur
% \begin{tabular}{|c|c|cccc|}
% \hline
% \multirow{2}{*}{Clean}     & ResNet50  \cite{He2015DeepRL}            & \multicolumn{1}{c|}{Adv-T$\star$ \cite{madry2018towards} } & \multicolumn{1}{c|}{CutMix \cite{CutMix}} & \multicolumn{1}{c|}{FALcon \cite{ibrayev2023exploring}} & GFNet \cite{huang2022glance}\\ \cline{2-6} 
%                            & 76.15                   & \multicolumn{1}{c|}{47.91} & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{72.97}  & 75.88   \\ 
%                            \hline
%                            \hline
% \multirow{2}{*}{Surrogate} & \multirow{2}{*}{Target} & \multicolumn{4}{c|}{Attack}                                                                      \\ \cline{3-6} 
%                            &                         & \multicolumn{1}{c|}{PGD \cite{madry2018towards}}   & \multicolumn{1}{c|}{MIM \cite{MIM}}    & \multicolumn{1}{c|}{VMI \cite{VMI}}    & P-IFGSM \cite{GaoZhang2020PatchWise} \\ \hline
% \multirow{5}{*}{ResNet34 \cite{He2015DeepRL}}  & ResNet50       & \multicolumn{1}{c|}{31.46} & \multicolumn{1}{c|}{20.20}  & \multicolumn{1}{c|}{11.61}  & 31.62   \\ \cline{2-6} 
%                            & Adv-T $\star$                  & \multicolumn{1}{c|}{47.63} & \multicolumn{1}{c|}{47.37}  & \multicolumn{1}{c|}{47.16}  & 46.94   \\ \cline{2-6} 
%                            & R-Blur                  & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}       &         \\ \cline{2-6} 
%                            & FALcon                  & \multicolumn{1}{c|}{49.83} & \multicolumn{1}{c|}{37.01}  & \multicolumn{1}{c|}{29.40}  & 40.46   \\ \cline{2-6} 
%                            & GFNet                  & \multicolumn{1}{c|}{57.82} & \multicolumn{1}{c|}{48.60}  & \multicolumn{1}{c|}{41.17}  & 46.93   \\ \hline
%                            \hline
% \multirow{5}{*}{ResNet50 \cite{He2015DeepRL}}  & ResNet50               & \multicolumn{1}{c|}{0.00}  & \multicolumn{1}{c|}{0.00}   & \multicolumn{1}{c|}{0.00}   & 0.00    \\ \cline{2-6} 
%                            & Adv-T $\star$                  & \multicolumn{1}{c|}{47.68} & \multicolumn{1}{c|}{47.36}  & \multicolumn{1}{c|}{47.22}  & 46.83   \\ \cline{2-6} 
%                            & R-Blur                  & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{}       &         \\ \cline{2-6} 
%                            & FALcon                  & \multicolumn{1}{c|}{37.54} & \multicolumn{1}{c|}{19.96}  & \multicolumn{1}{c|}{12.07}  &   27.37      \\ \cline{2-6} 
%                            & GFNet                   & \multicolumn{1}{c|}{51.85} & \multicolumn{1}{c|}{42.16}  & \multicolumn{1}{c|}{32.33}  & 43.33   \\ \hline

% \end{tabular}
\vspace{-7mm}
\end{table}

==> Tables_App/Multiple_Inference.tex <==
\begin{table}[t!]
\caption{Effects of Inference from Multiple Fixation Points}
\label{tab:multiple_pred}
\begin{tabular}{|c|c|cc|}
\hline
\multirow{2}{*}{Surrogate} & \multirow{2}{*}{Target} & \multicolumn{2}{c|}{Attack}                          \\ \cline{3-4} 
                           &                         & \multicolumn{1}{c|}{PGD}            & MIM            \\ \hline
\multirow{3}{*}{ResNet34}  & ResNet50                & \multicolumn{1}{c|}{31.46}          & 20.20          \\ \cline{2-4} 
                           & FALcon (Top-1)          & \multicolumn{1}{c|}{49.83}          & 37.01          \\ \cline{2-4} 
                           & FALcon (Any)            & \multicolumn{1}{c|}{\textbf{54.37}} & \textbf{41.40} \\ \hline
\end{tabular}
\end{table}

==> Tables_App/Token_Gradient_Regularization.tex <==
\begin{table}[t!]
\centering
\caption{Token Gradient Regularization.}
\label{tab:TGR-table}
\begin{tabular}{|c|c|ccc|}
\hline
\multirow{2}{*}{Target} & \multirow{2}{*}{Clean} & \multicolumn{3}{c|}{Surrogate}                                                             \\ \cline{3-5} 
                        &                        & \multicolumn{1}{c|}{ViT-B/16 \cite{dosovitskiy2021an}}       & \multicolumn{1}{c|}{CaiT-S/24 \cite{Touvron2021GoingDW}}      & PiT-B \cite{Heo2021RethinkingSD}         \\ \hline \hline
ResNet50 \cite{He2015DeepRL}                & \textbf{93.10}                  & \multicolumn{1}{c|}{32.0}           & \multicolumn{1}{c|}{13.3}           & 10.30          \\ \hline
Adv-T \cite{madry2018towards}                  & 28.80                  & \multicolumn{1}{c|}{27.70}          & \multicolumn{1}{c|}{26.90}          & 26.90          \\ \hline
%R-Blur \cite{shah2023training}                 &                        & \multicolumn{1}{c|}{}               & \multicolumn{1}{c|}{}               &                \\ \hline
Swin-v2 \cite{SwinV2}                & 99.00                  & \multicolumn{1}{c|}{31.10}          & \multicolumn{1}{c|}{10.3}           & 12.30          \\ \hline
RVT \cite{Mao2021TowardsRV}                    & 97.70                  & \multicolumn{1}{c|}{34.40}          & \multicolumn{1}{c|}{12.1}           & \textbf{14.50} \\ \hline
Adv-RVT \cite{Mao2021TowardsRV}               & 53.40                  & \multicolumn{1}{c|}{47.80}          & \multicolumn{1}{c|}{46.30}          & 45.70          \\ \hline
Focal Net  \cite{yang2022focal}             & \textbf{99.20}         & \multicolumn{1}{c|}{\textbf{35.60}} & \multicolumn{1}{c|}{13.20}          & 7.00           \\ \hline
FALcon \cite{ibrayev2023exploring}                 & 85.4                   & \multicolumn{1}{c|}{21.00}          & \multicolumn{1}{c|}{\textbf{15.10}} & 10.50          \\ \hline
GFNet  \cite{huang2022glance}                 & 89.5                   & \multicolumn{1}{c|}{\textbf{35.00}} & \multicolumn{1}{c|}{\textbf{22.5}}  & \textbf{15.80} \\ \hline
\end{tabular}
\end{table}

